An Empirical Study of Automated Unit Test Generation for Python

Various mature automated test generation tools exist for statically typed programming languages such as Java. Automatically generating unit tests for dynamically typed programming languages such as Python, however, is substantially more difficult due to the dynamic nature of these languages as well as the lack of type information. Our Pynguin framework provides automated unit test generation for Python. In this paper, we extend our previous work on Pynguin to support more aspects of the Python language, and by studying a larger variety of well-established state of the art test-generation algorithms, namely DynaMOSA, MIO, and MOSA. Furthermore, we improved our Pynguin tool to generate regression assertions, whose quality we also evaluate. Our experiments confirm that evolutionary algorithms can outperform random test generation also in the context of Python, and similar to the Java world, DynaMOSA yields the highest coverage results. However, our results also demonstrate that there are still fundamental remaining issues, such as inferring type information for code without this information, currently limiting the effectiveness of test generation for Python.

==> algorithms/random-tc.tex <==
\begin{algorithm}[t]
  \caption{\label{alg:random-tc}Random sampling on test-case level}

  \SetKwInput{Input}{Input}
  \SetKwInput{Output}{Output}

  \Input{Stopping condition~\(C\), Fitness function~\(\delta\)}
  %
  \Output{Archive of optimised individuals~\(A\)}
  %
  \(N \leftarrow \textsc{SampleTestCase}() \)\;
  \(A \leftarrow \{\} \)\;
  \(\textsc{PerformFitnessEvaluation}(\delta, N)\)\;
  \(\textsc{UpdateArchive}(A, N)\)\;
  %
  \While{\(\neg C\)}{%
    \(N \leftarrow \textsc{SampleTestCase}() \)\;
    \(\textsc{PerformFitnessEvaluation}(\delta, N)\)\;
    \(\textsc{UpdateArchive}(A, N)\)\;
  }
  %
  \Return{\(A\)}

\end{algorithm}



==> algorithms/random-ts.tex <==
\begin{algorithm}[t]
  \caption{\label{alg:random-ts}Random sampling on test-suite level}

  \SetKwInput{Input}{Input}
  \SetKwInput{Output}{Output}

  \Input{Stopping condition~\(C\), Fitness function~\(\delta\)}
  %
  \Output{Test suite~\(N\)}
  %
  \(N \leftarrow \textsc{SampleTestSuite}()\)\;
  \(f \leftarrow \textsc{PerformFitnessEvaluation}(\delta, N)\)\;
  \While{\(\neg C\)}{%
    \(N' \leftarrow \textsc{SampleTestSuite}()\)\;
    \(f' \leftarrow \textsc{PerformFitnessEvaluation}(\delta, N')\)\;
    \If{\(f' < f\)}{%
      \(N \leftarrow N'\)\;
      \(f \leftarrow f'\)\;
    }
  }
  \Return{N}

\end{algorithm}



==> generated/tables/algorithm-iterations.tex <==
\begin{longtable}{@{} l r r r r r @{}}
\caption{Overview over algorithm iterations. The table shows the mean number of algorithm iterations together with its standard deviation. For each module and algorithm, the upper row reports the results for the configuration with type information, the lower row reports the results for the configuration without type information.}\label{tab:algorithm-iterations}\\
\toprule
Module Name & DynaMOSA & MIO & MOSA & Random & WS \\ \midrule
\endfirsthead
\multicolumn{6}{@{}l}{\small\ldots\emph{continued}} \\ \toprule
Module Name & DynaMOSA & MIO & MOSA & Random & WS \\ \midrule
\endhead
\bottomrule
\multicolumn{6}{r@{}}{\small\emph{continued on next page} \ldots} \\
\endfoot
\bottomrule
\endlastfoot
\texttt{apimd.compiler} & \(\num{653.5} \pm \num{518.2410403104611}\) & \(\num{36582.03333333333} \pm \num{19675.105708839867}\) & \(\num{513.1333333333333} \pm \num{459.76963747101644}\) & \(\num{1821.8666666666666} \pm \num{114.57710348790529}\) & \(\num{437.5} \pm \num{130.21752358371688}\) \\
 & \(\num{1804.6666666666667} \pm \num{968.3632950831872}\) & \(\num{80901.53333333334} \pm \num{41237.052030770894}\) & \(\num{1246.1333333333334} \pm \num{582.0709598484111}\) & \(\num{1962.4} \pm \num{72.91733628592368}\) & \(\num{670.2} \pm \num{145.60418713191194}\) \\
\rowcolor{gray!25}
\texttt{codetiming.\_timer} & \(\num{267.6666666666667} \pm \num{365.3656018134517}\) & \(\num{5600.566666666667} \pm \num{4819.6512728572}\) & \(\num{193.86666666666667} \pm \num{219.42475473042177}\) & \(\num{1682.5} \pm \num{339.2885812686751}\) & \(\num{260.8333333333333} \pm \num{254.4557523127694}\) \\
\rowcolor{gray!25}
 & \(\num{79.76666666666667} \pm \num{89.64707943137195}\) & \(\num{5707.133333333333} \pm \num{7259.462798275107}\) & \(\num{105.4} \pm \num{233.4878864169366}\) & \(\num{1546.8333333333333} \pm \num{371.29401708947154}\) & \(\num{289.03333333333336} \pm \num{285.70137331249157}\) \\
\texttt{dataclasses\_json.api} & \(\num{5992.6} \pm \num{1021.9837572094773}\) & \(\num{552521.0} \pm \num{8387.751611930833}\) & \(\num{5617.6} \pm \num{863.8717018408344}\) & \(\num{2122.1} \pm \num{111.13345503306468}\) & \(\num{1642.4666666666667} \pm \num{573.7197281223487}\) \\
 & \(\num{4681.933333333333} \pm \num{1020.9860660784931}\) & \(\num{545317.5666666667} \pm \num{8433.04430932202}\) & \(\num{4048.1} \pm \num{907.2529339753587}\) & \(\num{2077.5666666666666} \pm \num{90.40929282924989}\) & \(\num{1801.8} \pm \num{616.8177733473975}\) \\
\rowcolor{gray!25}
\texttt{dataclasses\_json.mm} & \(\num{3222.6} \pm \num{307.8086732214426}\) & \(\num{180715.56666666668} \pm \num{5035.1883687897325}\) & \(\num{2076.9} \pm \num{323.4687374970432}\) & \(\num{2940.266666666667} \pm \num{147.38711246082622}\) & \(\num{974.3666666666667} \pm \num{214.3468802139916}\) \\
\rowcolor{gray!25}
 & \(\num{2804.9333333333334} \pm \num{246.22206592246445}\) & \(\num{196759.73333333334} \pm \num{4114.914336338279}\) & \(\num{1378.4333333333334} \pm \num{174.15622858233635}\) & \(\num{4222.6} \pm \num{177.06546617097538}\) & \(\num{1252.0} \pm \num{266.0439424424936}\) \\
\texttt{dataclasses\_json.undefined} & \(\num{3686.5666666666666} \pm \num{152.38578160964235}\) & \(\num{354511.4666666667} \pm \num{4610.840515293417}\) & \(\num{2467.0333333333333} \pm \num{110.45938037416143}\) & \(\num{1962.5333333333333} \pm \num{71.37793213173312}\) & \(\num{1491.6} \pm \num{401.2214626225341}\) \\
 & \(\num{1922.0} \pm \num{131.08486327303524}\) & \(\num{347157.8333333333} \pm \num{6923.706701507925}\) & \(\num{1284.9} \pm \num{101.1746015559241}\) & \(\num{2521.866666666667} \pm \num{166.8271319480827}\) & \(\num{1706.2} \pm \num{412.70482062306615}\) \\
\rowcolor{gray!25}
\texttt{docstring\_parser.google} & \(\num{3657.133333333333} \pm \num{1105.3432524546963}\) & \(\num{170726.8} \pm \num{11684.364027076585}\) & \(\num{1439.4333333333334} \pm \num{453.2040480792314}\) & \(\num{1983.6} \pm \num{62.28499570245768}\) & \(\num{1248.9333333333334} \pm \num{414.0252310596819}\) \\
\rowcolor{gray!25}
 & \(\num{2848.4333333333334} \pm \num{630.35275747043}\) & \(\num{185392.36666666667} \pm \num{6351.9123402453315}\) & \(\num{915.9333333333333} \pm \num{203.37258712865483}\) & \(\num{3078.0666666666666} \pm \num{164.6632788520223}\) & \(\num{1962.7} \pm \num{852.0569897566145}\) \\
\texttt{docstring\_parser.numpydoc} & \(\num{2294.9333333333334} \pm \num{951.8913634528324}\) & \(\num{172859.83333333334} \pm \num{12979.44217515379}\) & \(\num{2085.1666666666665} \pm \num{849.8134514697038}\) & \(\num{1490.9} \pm \num{34.67220888500641}\) & \(\num{820.5333333333333} \pm \num{200.52134349091696}\) \\
 & \(\num{2743.266666666667} \pm \num{634.8162337044578}\) & \(\num{255759.93333333332} \pm \num{10376.894027143899}\) & \(\num{2222.1666666666665} \pm \num{563.626440444215}\) & \(\num{1681.5} \pm \num{36.01604048772981}\) & \(\num{1384.6333333333334} \pm \num{261.11557532663755}\) \\
\rowcolor{gray!25}
\texttt{docstring\_parser.parser} & \(\num{5979.366666666667} \pm \num{2414.2676976863922}\) & \(\num{478093.1} \pm \num{23340.864050947806}\) & \(\num{6157.333333333333} \pm \num{2684.315790731004}\) & \(\num{1506.6666666666667} \pm \num{32.24511011667942}\) & \(\num{1989.2666666666667} \pm \num{878.9720458986534}\) \\
\rowcolor{gray!25}
 & \(\num{11151.466666666667} \pm \num{1855.4840382207424}\) & \(\num{555678.6333333333} \pm \num{10393.233231235146}\) & \(\num{11316.933333333332} \pm \num{1921.0553481289166}\) & \(\num{2768.8} \pm \num{66.03990434212666}\) & \(\num{2511.2} \pm \num{735.6873117633979}\) \\
\texttt{docstring\_parser.rest} & \(\num{1857.0333333333333} \pm \num{314.3775989358079}\) & \(\num{113853.96666666666} \pm \num{3389.8076080421188}\) & \(\num{1246.0} \pm \num{157.3386420300559}\) & \(\num{1527.8666666666666} \pm \num{38.26741959289717}\) & \(\num{1193.6333333333334} \pm \num{294.4441265811918}\) \\
 & \(\num{2640.3} \pm \num{691.2462084450484}\) & \(\num{156428.36666666667} \pm \num{7779.304452036265}\) & \(\num{1799.2} \pm \num{465.696763851832}\) & \(\num{2435.9666666666667} \pm \num{86.55414224766996}\) & \(\num{1900.9333333333334} \pm \num{753.5991312194519}\) \\
\rowcolor{gray!25}
\texttt{flake8.exceptions} & \(\num{0.13333333333333333} \pm \num{0.43417248545530474}\) & \(\num{41.8} \pm \num{44.22778031649495}\) & \(\num{0.13333333333333333} \pm \num{0.43417248545530474}\) & \(\num{46.36666666666667} \pm \num{33.65595026894571}\) & \(\num{0.03333333333333333} \pm \num{0.18257418583505533}\) \\
\rowcolor{gray!25}
 & \(\num{0.23333333333333334} \pm \num{0.6789105539243627}\) & \(\num{43.06666666666667} \pm \num{31.90928233054725}\) & \(\num{0.23333333333333334} \pm \num{0.6789105539243627}\) & \(\num{81.16666666666667} \pm \num{96.58659981782056}\) & \(\num{0.06666666666666667} \pm \num{0.2537081317024625}\) \\
\texttt{flake8.formatting.base} & \(\num{2158.9} \pm \num{24.3244590966547}\) & \(\num{480442.6666666667} \pm \num{8359.280707933127}\) & \(\num{1725.8} \pm \num{18.82661359114657}\) & \(\num{11308.3} \pm \num{240.89604998121436}\) & \(\num{5166.033333333334} \pm \num{4190.180668340367}\) \\
 & \(\num{2149.0666666666666} \pm \num{35.985565433104284}\) & \(\num{477641.0333333333} \pm \num{7394.878113207506}\) & \(\num{1734.5333333333333} \pm \num{19.11441653674602}\) & \(\num{10970.2} \pm \num{120.20998868359626}\) & \(\num{5151.7} \pm \num{4190.342617462698}\) \\
\rowcolor{gray!25}
\texttt{flake8.formatting.default} & \(\num{4956.7} \pm \num{71.16815928876989}\) & \(\num{619225.4} \pm \num{12226.710761336399}\) & \(\num{4962.4} \pm \num{78.2892955205464}\) & \(\num{11371.8} \pm \num{199.5096402475934}\) & \(\num{5196.766666666666} \pm \num{4152.853382861022}\) \\
\rowcolor{gray!25}
 & \(\num{4986.166666666667} \pm \num{83.02599648275246}\) & \(\num{619902.3666666667} \pm \num{9456.124556050445}\) & \(\num{5013.666666666667} \pm \num{66.81747310878853}\) & \(\num{11041.966666666667} \pm \num{117.82643088921922}\) & \(\num{5298.433333333333} \pm \num{4403.10211714684}\) \\
\texttt{flake8.main.debug} & \(\num{5683.033333333334} \pm \num{472.9206744981828}\) & \(\num{577402.6666666666} \pm \num{17720.13595404632}\) & \(\num{5748.333333333333} \pm \num{461.30686423302404}\) & \(\num{10493.833333333334} \pm \num{284.65430738466563}\) & \(\num{1932.5333333333333} \pm \num{562.3459932212144}\) \\
 & \(\num{4567.266666666666} \pm \num{355.29210258732115}\) & \(\num{594794.5} \pm \num{17357.7094066247}\) & \(\num{4540.466666666666} \pm \num{362.16215965373505}\) & \(\num{10169.866666666667} \pm \num{156.56148584685414}\) & \(\num{2045.0} \pm \num{629.4786567552111}\) \\
\rowcolor{gray!25}
\texttt{flake8.main.git} & \(\num{2446.633333333333} \pm \num{654.8618429358465}\) & \(\num{270897.6} \pm \num{5972.690051825259}\) & \(\num{2025.1} \pm \num{505.1214500596315}\) & \(\num{2884.4666666666667} \pm \num{367.81383347007767}\) & \(\num{987.7333333333333} \pm \num{294.34942094251755}\) \\
\rowcolor{gray!25}
 & \(\num{2181.5333333333333} \pm \num{703.6722264654551}\) & \(\num{272120.23333333334} \pm \num{5521.042715630454}\) & \(\num{2005.9} \pm \num{465.71356817920486}\) & \(\num{2850.766666666667} \pm \num{422.11484655027346}\) & \(\num{1018.5333333333333} \pm \num{258.0137303661789}\) \\
\texttt{flutes.math} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0666666666666667} \pm \num{0.36514837167011066}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.1} \pm \num{0.40257789993644877}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{flutes.timing} & \(\num{6935.233333333334} \pm \num{325.2440657396389}\) & \(\num{1222641.5333333334} \pm \num{19043.933545309406}\) & \(\num{7142.766666666666} \pm \num{400.2890923710816}\) & \(\num{1492.8} \pm \num{39.385276436759966}\) & \(\num{5110.433333333333} \pm \num{5165.060480891232}\) \\
\rowcolor{gray!25}
 & \(\num{8173.2} \pm \num{383.30076423360936}\) & \(\num{1175298.3333333333} \pm \num{21492.121339648187}\) & \(\num{8117.733333333334} \pm \num{407.8330399878695}\) & \(\num{1460.9} \pm \num{33.85603394496701}\) & \(\num{5510.433333333333} \pm \num{5456.5586330664455}\) \\
\texttt{flutils.decorators} & \(\num{8642.733333333334} \pm \num{153.82702630873584}\) & \(\num{642274.5} \pm \num{12804.47102342206}\) & \(\num{8758.133333333333} \pm \num{142.35791060788887}\) & \(\num{1972.4666666666667} \pm \num{70.70225735718981}\) & \(\num{2743.1666666666665} \pm \num{1542.7739925063631}\) \\
 & \(\num{8773.666666666666} \pm \num{111.81583791751238}\) & \(\num{639586.3} \pm \num{13120.412998519678}\) & \(\num{8790.066666666668} \pm \num{156.45775750999843}\) & \(\num{1927.2} \pm \num{73.5627341938088}\) & \(\num{2915.1} \pm \num{1465.576415965569}\) \\
\rowcolor{gray!25}
\texttt{flutils.namedtupleutils} & \(\num{5671.333333333333} \pm \num{1625.943510350398}\) & \(\num{247333.96666666667} \pm \num{15770.78226796877}\) & \(\num{5433.466666666666} \pm \num{1405.8687517426497}\) & \(\num{1380.7333333333333} \pm \num{43.56678055372111}\) & \(\num{1505.9} \pm \num{430.8710784061708}\) \\
\rowcolor{gray!25}
 & \(\num{6738.033333333334} \pm \num{2320.233972793638}\) & \(\num{273611.23333333334} \pm \num{10479.183837932962}\) & \(\num{7102.233333333334} \pm \num{2041.3002057230722}\) & \(\num{1465.5} \pm \num{62.36032668955148}\) & \(\num{1650.0333333333333} \pm \num{751.2090706428485}\) \\
\texttt{flutils.packages} & \(\num{5063.333333333333} \pm \num{263.05425339630045}\) & \(\num{333841.5} \pm \num{31227.9985399376}\) & \(\num{1426.2666666666667} \pm \num{76.87200886620849}\) & \(\num{14865.366666666667} \pm \num{288.42264047787563}\) & \(\num{4666.766666666666} \pm \num{3890.4929187154057}\) \\
 & \(\num{3919.233333333333} \pm \num{254.20853282476483}\) & \(\num{357564.6} \pm \num{4133.716926397623}\) & \(\num{1083.7} \pm \num{73.878348281669}\) & \(\num{5554.4} \pm \num{612.1561441557099}\) & \(\num{5521.3} \pm \num{4695.89566316271}\) \\
\rowcolor{gray!25}
\texttt{flutils.pathutils} & \(\num{1424.7333333333333} \pm \num{360.3214018673859}\) & \(\num{119803.23333333334} \pm \num{7646.892385183324}\) & \(\num{868.8666666666667} \pm \num{150.24273080891314}\) & \(\num{3427.3} \pm \num{608.0108977017912}\) & \(\num{705.1333333333333} \pm \num{128.85750840080823}\) \\
\rowcolor{gray!25}
 & \(\num{2991.133333333333} \pm \num{637.7474223488824}\) & \(\num{124351.76666666666} \pm \num{4741.016373524034}\) & \(\num{1917.2333333333333} \pm \num{589.4048244852062}\) & \(\num{3597.2} \pm \num{826.7876098032299}\) & \(\num{716.9} \pm \num{175.4364704741115}\) \\
\texttt{flutils.setuputils.cmd} & \(\num{5042.766666666666} \pm \num{308.59623026429426}\) & \(\num{545767.7} \pm \num{11394.556934540402}\) & \(\num{2707.9333333333334} \pm \num{161.10200951963438}\) & \(\num{1524.9333333333334} \pm \num{118.34576266275815}\) & \(\num{2651.6} \pm \num{1112.6803797974542}\) \\
 & \(\num{4528.466666666666} \pm \num{44.469852890379045}\) & \(\num{520686.5} \pm \num{8936.793653785726}\) & \(\num{2046.7333333333333} \pm \num{28.992190783671067}\) & \(\num{11675.333333333334} \pm \num{3886.929550858021}\) & \(\num{4904.633333333333} \pm \num{4004.654537456111}\) \\
\rowcolor{gray!25}
\texttt{flutils.strutils} & \(\num{31.1} \pm \num{33.924205578582544}\) & \(\num{1380.9} \pm \num{1828.2726603790952}\) & \(\num{25.266666666666666} \pm \num{29.123912835513273}\) & \(\num{1254.6666666666667} \pm \num{446.8113335806198}\) & \(\num{34.166666666666664} \pm \num{55.065530449439606}\) \\
\rowcolor{gray!25}
 & \(\num{440.5} \pm \num{403.1938654089969}\) & \(\num{42525.96666666667} \pm \num{39803.29722738135}\) & \(\num{932.2666666666667} \pm \num{636.9610464641017}\) & \(\num{1460.8333333333333} \pm \num{75.57142469138091}\) & \(\num{930.3} \pm \num{653.8046818958743}\) \\
\texttt{httpie.cli.dicts} & \(\num{91.8} \pm \num{106.82289564734126}\) & \(\num{3269.0666666666666} \pm \num{2203.640341349511}\) & \(\num{126.83333333333333} \pm \num{161.1390668043436}\) & \(\num{1630.5333333333333} \pm \num{38.52069155870543}\) & \(\num{130.53333333333333} \pm \num{134.24314875816103}\) \\
 & \(\num{55.233333333333334} \pm \num{33.07325550781261}\) & \(\num{2867.9} \pm \num{1447.6730281910084}\) & \(\num{85.43333333333334} \pm \num{76.02253900509774}\) & \(\num{1632.5} \pm \num{30.692861126619185}\) & \(\num{269.1666666666667} \pm \num{326.14848356742874}\) \\
\rowcolor{gray!25}
\texttt{httpie.cli.exceptions} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{httpie.config} & \(\num{2752.6666666666665} \pm \num{534.2767159397855}\) & \(\num{328256.4666666667} \pm \num{6236.617964632884}\) & \(\num{2748.0333333333333} \pm \num{415.3787206985878}\) & \(\num{1919.0333333333333} \pm \num{204.0348995389883}\) & \(\num{1415.2333333333333} \pm \num{287.9416467863289}\) \\
 & \(\num{3120.9666666666667} \pm \num{621.7434044037301}\) & \(\num{341412.3} \pm \num{7895.864828481753}\) & \(\num{3071.1666666666665} \pm \num{447.24344087118686}\) & \(\num{1880.2666666666667} \pm \num{130.3739801979048}\) & \(\num{1338.7333333333333} \pm \num{327.016179430308}\) \\
\rowcolor{gray!25}
\texttt{httpie.models} & \(\num{1928.1} \pm \num{84.29437335498939}\) & \(\num{421852.26666666666} \pm \num{11731.455511111799}\) & \(\num{1821.5} \pm \num{64.41500681866204}\) & \(\num{1765.3666666666666} \pm \num{67.21170019928198}\) & \(\num{1786.0666666666666} \pm \num{502.3972829196606}\) \\
\rowcolor{gray!25}
 & \(\num{1930.8333333333333} \pm \num{56.22374227497044}\) & \(\num{410654.0} \pm \num{9540.884604400306}\) & \(\num{1835.8666666666666} \pm \num{46.16741150484258}\) & \(\num{1775.9333333333334} \pm \num{52.879129142323954}\) & \(\num{1862.9} \pm \num{516.7255224171159}\) \\
\texttt{httpie.output.formatters.colors} & \(\num{4035.1666666666665} \pm \num{849.7920671971847}\) & \(\num{318906.9666666667} \pm \num{27452.42171276338}\) & \(\num{4036.8} \pm \num{930.7842966533931}\) & \(\num{2766.6} \pm \num{153.63247681084388}\) & \(\num{1745.2666666666667} \pm \num{679.6285970182961}\) \\
 & \(\num{2999.233333333333} \pm \num{669.4714169857587}\) & \(\num{419326.0} \pm \num{12767.851835087946}\) & \(\num{2070.1} \pm \num{1055.5344895457893}\) & \(\num{3534.366666666667} \pm \num{85.84849659613202}\) & \(\num{3115.4666666666667} \pm \num{1599.45007216022}\) \\
\rowcolor{gray!25}
\texttt{httpie.output.formatters.headers} & \(\num{8176.666666666667} \pm \num{472.1512274782259}\) & \(\num{856672.1333333333} \pm \num{25014.549473474828}\) & \(\num{8297.8} \pm \num{532.7794652768532}\) & \(\num{15052.2} \pm \num{290.6525832294133}\) & \(\num{5270.566666666667} \pm \num{4882.142531952427}\) \\
\rowcolor{gray!25}
 & \(\num{7758.666666666667} \pm \num{535.2359024433691}\) & \(\num{882941.4} \pm \num{20226.402868698544}\) & \(\num{7766.033333333334} \pm \num{629.7612839105336}\) & \(\num{16889.6} \pm \num{216.1939742054774}\) & \(\num{5528.666666666667} \pm \num{4872.761868784997}\) \\
\texttt{httpie.output.formatters.json} & \(\num{6854.8} \pm \num{425.547387855154}\) & \(\num{750976.0666666667} \pm \num{25161.564457053082}\) & \(\num{5469.333333333333} \pm \num{292.922648767417}\) & \(\num{14465.933333333332} \pm \num{262.0761844135816}\) & \(\num{4835.333333333333} \pm \num{4677.489839155432}\) \\
 & \(\num{5309.5} \pm \num{396.77629847873067}\) & \(\num{734564.2666666667} \pm \num{15481.690952671253}\) & \(\num{4154.6} \pm \num{260.6492689023131}\) & \(\num{16424.433333333334} \pm \num{191.52755871447442}\) & \(\num{4852.933333333333} \pm \num{3603.891200980649}\) \\
\rowcolor{gray!25}
\texttt{httpie.output.processing} & \(\num{5580.7} \pm \num{869.5270275984168}\) & \(\num{433018.6} \pm \num{17712.960930853176}\) & \(\num{5689.066666666667} \pm \num{896.5423594559549}\) & \(\num{1702.4} \pm \num{155.90726686742013}\) & \(\num{1648.0666666666666} \pm \num{711.1616496648444}\) \\
\rowcolor{gray!25}
 & \(\num{5772.233333333334} \pm \num{1476.8326705424718}\) & \(\num{439434.4666666667} \pm \num{11174.258286681548}\) & \(\num{4797.0} \pm \num{1157.1530760358849}\) & \(\num{2495.633333333333} \pm \num{266.28173870510926}\) & \(\num{1830.0} \pm \num{486.2746492289708}\) \\
\texttt{httpie.output.streams} & \(\num{4204.6} \pm \num{715.6197506960012}\) & \(\num{343883.93333333335} \pm \num{7842.450179821896}\) & \(\num{2315.2} \pm \num{421.3111226504298}\) & \(\num{2813.9} \pm \num{96.66342245844243}\) & \(\num{1588.0} \pm \num{582.4723169387538}\) \\
 & \(\num{4876.9} \pm \num{814.8036509829667}\) & \(\num{343396.76666666666} \pm \num{5663.624943038009}\) & \(\num{3081.8333333333335} \pm \num{555.9529925138072}\) & \(\num{3120.2} \pm \num{100.2346901199793}\) & \(\num{1830.9666666666667} \pm \num{595.5607895278101}\) \\
\rowcolor{gray!25}
\texttt{httpie.plugins.base} & \(\num{8150.166666666667} \pm \num{778.2361614500483}\) & \(\num{603911.0333333333} \pm \num{18756.948925634217}\) & \(\num{8289.966666666667} \pm \num{778.2543012867095}\) & \(\num{2505.2} \pm \num{112.93006685555446}\) & \(\num{1880.0666666666666} \pm \num{470.5597498309004}\) \\
\rowcolor{gray!25}
 & \(\num{6769.833333333333} \pm \num{708.572829018294}\) & \(\num{649134.6666666666} \pm \num{12972.494417123442}\) & \(\num{6783.266666666666} \pm \num{741.4082096479194}\) & \(\num{2834.6666666666665} \pm \num{103.64339835700345}\) & \(\num{2180.9333333333334} \pm \num{708.4143991475189}\) \\
\texttt{httpie.plugins.manager} & \(\num{5583.266666666666} \pm \num{1603.6273092980289}\) & \(\num{458737.1666666667} \pm \num{11007.457726103426}\) & \(\num{5732.266666666666} \pm \num{1558.306019552871}\) & \(\num{1770.5333333333333} \pm \num{100.06505929621}\) & \(\num{1520.6666666666667} \pm \num{300.4213516142738}\) \\
 & \(\num{5019.433333333333} \pm \num{1471.3806718892279}\) & \(\num{461880.6666666667} \pm \num{9205.637104825886}\) & \(\num{5104.433333333333} \pm \num{1277.5715563557276}\) & \(\num{2115.8} \pm \num{80.85892354738208}\) & \(\num{1772.7} \pm \num{624.5772722133886}\) \\
\rowcolor{gray!25}
\texttt{httpie.sessions} & \(\num{3231.3333333333335} \pm \num{577.4423591674927}\) & \(\num{288247.8333333333} \pm \num{9601.891573999914}\) & \(\num{3004.2} \pm \num{739.3057041156459}\) & \(\num{2604.4666666666667} \pm \num{123.26470908474624}\) & \(\num{1367.4} \pm \num{375.12366696496423}\) \\
\rowcolor{gray!25}
 & \(\num{4529.8} \pm \num{1118.8168442754527}\) & \(\num{326009.13333333336} \pm \num{9647.562649967993}\) & \(\num{3789.766666666667} \pm \num{941.2087490006678}\) & \(\num{2932.3333333333335} \pm \num{228.4081847276378}\) & \(\num{1626.2} \pm \num{560.4675634282258}\) \\
\texttt{httpie.ssl} & \(\num{0.0} \pm \num{0.0}\) & \(\num{11.0} \pm \num{7.969770472184901}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{6.866666666666666} \pm \num{3.4112727257132933}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.1} \pm \num{0.4025778999364487}\) & \(\num{20.4} \pm \num{15.178478411769467}\) & \(\num{0.1} \pm \num{0.4025778999364487}\) & \(\num{20.1} \pm \num{15.892635466434303}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{httpie.status} & \(\num{0.9666666666666667} \pm \num{2.092405534197477}\) & \(\num{94.16666666666667} \pm \num{82.81932280503781}\) & \(\num{0.7} \pm \num{1.2635472781569874}\) & \(\num{245.06666666666666} \pm \num{292.979454773778}\) & \(\num{0.4666666666666667} \pm \num{0.7302967433402215}\) \\
\rowcolor{gray!25}
 & \(\num{47.56666666666667} \pm \num{33.74926137974224}\) & \(\num{867.9} \pm \num{629.6972096667324}\) & \(\num{41.56666666666667} \pm \num{26.61304234747515}\) & \(\num{1428.0666666666666} \pm \num{176.3112321286215}\) & \(\num{55.03333333333333} \pm \num{35.62107409301732}\) \\
\texttt{isort.comments} & \(\num{0.0} \pm \num{0.0}\) & \(\num{15.766666666666667} \pm \num{11.370510355614055}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{63.3} \pm \num{61.74147993713453}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{1.9666666666666666} \pm \num{4.03846448570479}\) & \(\num{109.7} \pm \num{101.82986148304029}\) & \(\num{2.1} \pm \num{4.4671212669674745}\) & \(\num{388.43333333333334} \pm \num{420.86812442963594}\) & \(\num{0.3333333333333333} \pm \num{1.1244411127720095}\) \\
\rowcolor{gray!25}
\texttt{isort.exceptions} & \(\num{8428.066666666668} \pm \num{2656.3755178728065}\) & \(\num{426595.1666666667} \pm \num{8204.87943588882}\) & \(\num{8473.6} \pm \num{2609.2265150608428}\) & \(\num{1543.9333333333334} \pm \num{37.80524806966878}\) & \(\num{1703.5666666666666} \pm \num{461.3370137219482}\) \\
\rowcolor{gray!25}
 & \(\num{6845.833333333333} \pm \num{2073.5545373923082}\) & \(\num{423843.06666666665} \pm \num{6091.46832949129}\) & \(\num{6822.433333333333} \pm \num{2106.12942398484}\) & \(\num{1492.5666666666666} \pm \num{27.936730652319177}\) & \(\num{1909.7666666666667} \pm \num{593.0852519595762}\) \\
\texttt{isort.utils} & \(\num{11100.633333333333} \pm \num{184.69629933625023}\) & \(\num{712534.7666666667} \pm \num{25736.028146098644}\) & \(\num{8118.066666666667} \pm \num{115.41228445143457}\) & \(\num{1561.8666666666666} \pm \num{33.419727122158555}\) & \(\num{4440.466666666666} \pm \num{3626.999583899782}\) \\
 & \(\num{11864.866666666667} \pm \num{227.6680483288884}\) & \(\num{717531.6} \pm \num{17547.63245372533}\) & \(\num{8769.266666666666} \pm \num{119.86772403098266}\) & \(\num{1470.0} \pm \num{34.500374810557716}\) & \(\num{3686.8} \pm \num{1990.4062555340217}\) \\
\rowcolor{gray!25}
\texttt{mimesis.builtins.base} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0333333333333334} \pm \num{0.18257418583505533}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.9666666666666666} \pm \num{2.0924055341974768}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.4666666666666666} \pm \num{0.7760791522613609}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{mimesis.builtins.da} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.2333333333333334} \pm \num{0.7738543627276672}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.9333333333333333} \pm \num{1.0806553992619585}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.5} \pm \num{1.2525835370311151}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{2.1333333333333333} \pm \num{1.3578211078487255}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{mimesis.builtins.de} & \(\num{0.0} \pm \num{0.0}\) & \(\num{5.633333333333334} \pm \num{4.88123312100633}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{17.6} \pm \num{20.50332185028933}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{5.2} \pm \num{6.5516515422475345}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{12.933333333333334} \pm \num{10.071925245995402}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{mimesis.builtins.it} & \(\num{0.0} \pm \num{0.0}\) & \(\num{7.8} \pm \num{6.920235196322}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{26.033333333333335} \pm \num{20.29010856913108}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{20.833333333333332} \pm \num{25.345996532586465}\) & \(\num{850.9} \pm \num{952.6769308022308}\) & \(\num{20.833333333333332} \pm \num{25.34599653258647}\) & \(\num{1185.7666666666667} \pm \num{504.86165283743543}\) & \(\num{18.533333333333335} \pm \num{31.66934047997814}\) \\
\rowcolor{gray!25}
\texttt{mimesis.builtins.nl} & \(\num{0.0} \pm \num{0.0}\) & \(\num{2.9} \pm \num{2.9166584564744875}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{6.833333333333333} \pm \num{3.8424429489703495}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{8.433333333333334} \pm \num{6.355466467773118}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{7.7} \pm \num{4.26007932579535}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{mimesis.builtins.pt\_br} & \(\num{1628.6333333333334} \pm \num{109.21237877713736}\) & \(\num{383176.4666666667} \pm \num{9347.491475158506}\) & \(\num{1616.5333333333333} \pm \num{109.97640290263314}\) & \(\num{1410.9333333333334} \pm \num{38.95260898998213}\) & \(\num{1892.7333333333333} \pm \num{707.7458112439334}\) \\
 & \(\num{3630.8} \pm \num{716.3610821366555}\) & \(\num{404008.2} \pm \num{4872.116493992574}\) & \(\num{3675.733333333333} \pm \num{796.9545452072138}\) & \(\num{1577.1} \pm \num{31.342765760494736}\) & \(\num{1823.1666666666667} \pm \num{604.8650509700965}\) \\
\rowcolor{gray!25}
\texttt{mimesis.builtins.uk} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.3333333333333333} \pm \num{1.3217891045025338}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{2.0} \pm \num{1.144702942944678}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.9666666666666666} \pm \num{1.7904600320690713}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{2.066666666666667} \pm \num{1.112106833535071}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{mimesis.decorators} & \(\num{3576.5666666666666} \pm \num{140.0880716409929}\) & \(\num{944303.3333333334} \pm \num{22299.356043483025}\) & \(\num{3236.9333333333334} \pm \num{125.82827195423334}\) & \(\num{1485.4} \pm \num{39.77835141605683}\) & \(\num{4380.266666666666} \pm \num{4345.181682907087}\) \\
 & \(\num{3958.9} \pm \num{237.51375277785638}\) & \(\num{940865.1333333333} \pm \num{28976.66573800295}\) & \(\num{3565.766666666667} \pm \num{193.84880054120626}\) & \(\num{1450.4666666666667} \pm \num{24.87033038247247}\) & \(\num{4482.166666666667} \pm \num{4821.344604863935}\) \\
\rowcolor{gray!25}
\texttt{mimesis.exceptions} & \(\num{0.03333333333333333} \pm \num{0.18257418583505533}\) & \(\num{28.0} \pm \num{14.703975535606828}\) & \(\num{0.03333333333333333} \pm \num{0.18257418583505533}\) & \(\num{164.76666666666668} \pm \num{184.32480390151875}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.16666666666666666} \pm \num{0.461133037377414}\) & \(\num{76.33333333333333} \pm \num{52.17697558894339}\) & \(\num{0.16666666666666666} \pm \num{0.461133037377414}\) & \(\num{391.76666666666665} \pm \num{312.3815840010235}\) & \(\num{0.6666666666666666} \pm \num{0.7111590022187596}\) \\
\texttt{mimesis.providers.choice} & \(\num{3717.4} \pm \num{1911.4309425861718}\) & \(\num{176030.1} \pm \num{30915.941106602215}\) & \(\num{3567.6} \pm \num{2175.7826748726225}\) & \(\num{1959.3} \pm \num{106.18628718533715}\) & \(\num{1127.6333333333334} \pm \num{362.14985308840596}\) \\
 & \(\num{4951.966666666666} \pm \num{1829.9547475718955}\) & \(\num{194832.53333333333} \pm \num{55093.155714057015}\) & \(\num{4840.0} \pm \num{1641.2725718698932}\) & \(\num{2428.9333333333334} \pm \num{174.04932581337957}\) & \(\num{1507.8666666666666} \pm \num{338.95302627796156}\) \\
\rowcolor{gray!25}
\texttt{mimesis.providers.clothing} & \(\num{0.0} \pm \num{0.0}\) & \(\num{2.466666666666667} \pm \num{1.7167196733251497}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{7.266666666666667} \pm \num{3.0164301043970245}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{6.6} \pm \num{4.20672696096834}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{8.833333333333334} \pm \num{4.579439307144063}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{mimesis.providers.code} & \(\num{0.0} \pm \num{0.0}\) & \(\num{15.4} \pm \num{7.504481419745828}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{22.3} \pm \num{8.650891921327116}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{25.966666666666665} \pm \num{15.52635875187592}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{24.9} \pm \num{8.906990667931604}\) & \(\num{0.03333333333333333} \pm \num{0.18257418583505533}\) \\
\rowcolor{gray!25}
\texttt{mimesis.providers.development} & \(\num{0.43333333333333335} \pm \num{0.858359836662575}\) & \(\num{47.766666666666666} \pm \num{24.759092141638813}\) & \(\num{0.5} \pm \num{0.7310832774866962}\) & \(\num{211.13333333333333} \pm \num{204.02192805293453}\) & \(\num{0.2} \pm \num{0.5508613944197477}\) \\
\rowcolor{gray!25}
 & \(\num{1.2666666666666666} \pm \num{0.9444331755018487}\) & \(\num{85.5} \pm \num{44.5016466181212}\) & \(\num{1.2} \pm \num{1.0635010497214474}\) & \(\num{236.9} \pm \num{181.4697371939503}\) & \(\num{2.1333333333333333} \pm \num{1.3829836145670416}\) \\
\texttt{mimesis.providers.hardware} & \(\num{0.0} \pm \num{0.0}\) & \(\num{6.766666666666667} \pm \num{4.746565606569793}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{46.53333333333333} \pm \num{16.596080412479065}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{29.7} \pm \num{15.99385657919509}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{74.93333333333334} \pm \num{28.529396011510816}\) & \(\num{0.1} \pm \num{0.30512857662936466}\) \\
\rowcolor{gray!25}
\texttt{mimesis.providers.numbers} & \(\num{0.0} \pm \num{0.0}\) & \(\num{11.866666666666667} \pm \num{7.528031905339941}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{31.3} \pm \num{14.591329499114334}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{1.8333333333333333} \pm \num{3.1849141528335636}\) & \(\num{91.63333333333334} \pm \num{64.65957716796662}\) & \(\num{1.9} \pm \num{3.187800019687126}\) & \(\num{129.4} \pm \num{90.74617879292352}\) & \(\num{1.4666666666666666} \pm \num{2.224213667070142}\) \\
\texttt{mimesis.providers.science} & \(\num{0.0} \pm \num{0.0}\) & \(\num{20.233333333333334} \pm \num{18.654172748196054}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{31.533333333333335} \pm \num{27.853970599555815}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{8.766666666666667} \pm \num{15.377285831388772}\) & \(\num{175.66666666666666} \pm \num{158.73037936492605}\) & \(\num{8.766666666666667} \pm \num{15.377285831388773}\) & \(\num{660.7666666666667} \pm \num{540.2096453410844}\) & \(\num{3.2} \pm \num{6.905270351020999}\) \\
\rowcolor{gray!25}
\texttt{mimesis.providers.transport} & \(\num{0.03333333333333333} \pm \num{0.18257418583505536}\) & \(\num{15.466666666666667} \pm \num{8.923944285415244}\) & \(\num{0.03333333333333333} \pm \num{0.18257418583505533}\) & \(\num{34.666666666666664} \pm \num{27.571015932319757}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.26666666666666666} \pm \num{0.6914918072835209}\) & \(\num{40.8} \pm \num{29.98781361682177}\) & \(\num{0.26666666666666666} \pm \num{0.6914918072835209}\) & \(\num{65.36666666666666} \pm \num{45.29328437191768}\) & \(\num{0.1} \pm \num{0.30512857662936466}\) \\
\texttt{mimesis.providers.units} & \(\num{0.0} \pm \num{0.0}\) & \(\num{13.233333333333333} \pm \num{16.641624865406612}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{27.466666666666665} \pm \num{14.68927202565458}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{14.033333333333333} \pm \num{12.408237901333612}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{28.666666666666668} \pm \num{18.83747792865711}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{mimesis.shortcuts} & \(\num{0.7} \pm \num{0.9523111632886269}\) & \(\num{68.46666666666667} \pm \num{46.48302124827748}\) & \(\num{0.8} \pm \num{1.2972118642263706}\) & \(\num{107.66666666666667} \pm \num{125.36521360253487}\) & \(\num{0.2} \pm \num{0.6102571532587293}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{15.633333333333333} \pm \num{16.62669920449581}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{36.13333333333333} \pm \num{47.838617594296494}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{pdir.\_internal\_utils} & \(\num{287.56666666666666} \pm \num{51.235550247805506}\) & \(\num{65106.333333333336} \pm \num{2997.5878731859157}\) & \(\num{286.23333333333335} \pm \num{50.153339582368474}\) & \(\num{1319.8} \pm \num{37.91769671456761}\) & \(\num{540.4333333333333} \pm \num{114.75842192318109}\) \\
 & \(\num{556.5666666666667} \pm \num{230.5234947010725}\) & \(\num{94686.9} \pm \num{2846.9325458622397}\) & \(\num{533.0666666666667} \pm \num{158.0257363005575}\) & \(\num{1424.9666666666667} \pm \num{56.126386525125746}\) & \(\num{1015.8666666666667} \pm \num{200.2122551854326}\) \\
\rowcolor{gray!25}
\texttt{pdir.attr\_category} & \(\num{836.6} \pm \num{390.8584363185466}\) & \(\num{69200.16666666667} \pm \num{9218.082447328574}\) & \(\num{822.3666666666667} \pm \num{426.9337737008361}\) & \(\num{1478.5} \pm \num{45.513734190901104}\) & \(\num{749.4333333333333} \pm \num{163.21102974335116}\) \\
\rowcolor{gray!25}
 & \(\num{1741.4333333333334} \pm \num{354.4197475751942}\) & \(\num{238432.73333333334} \pm \num{8632.414258273104}\) & \(\num{1635.7333333333333} \pm \num{432.9733553427758}\) & \(\num{1791.5} \pm \num{45.03619234226685}\) & \(\num{1402.4333333333334} \pm \num{345.6387074561442}\) \\
\texttt{pdir.color} & \(\num{5274.733333333334} \pm \num{270.83739024370874}\) & \(\num{424730.7} \pm \num{6738.492664510007}\) & \(\num{4783.266666666666} \pm \num{131.6918904981947}\) & \(\num{1460.7666666666667} \pm \num{50.92975780312584}\) & \(\num{2233.5} \pm \num{1012.8920271286025}\) \\
 & \(\num{6396.5} \pm \num{817.5982383239}\) & \(\num{442859.93333333335} \pm \num{14307.899438430153}\) & \(\num{5728.266666666666} \pm \num{212.475545584108}\) & \(\num{1516.5} \pm \num{38.549341422882065}\) & \(\num{2340.8333333333335} \pm \num{949.5569232935499}\) \\
\rowcolor{gray!25}
\texttt{pdir.configuration} & \(\num{2791.766666666667} \pm \num{180.80083981597244}\) & \(\num{281654.8333333333} \pm \num{5498.320389827733}\) & \(\num{1667.0666666666666} \pm \num{74.89207560553885}\) & \(\num{46738.5} \pm \num{1884.2022870755384}\) & \(\num{3280.8333333333335} \pm \num{2198.4117634349564}\) \\
\rowcolor{gray!25}
 & \(\num{2814.266666666667} \pm \num{182.91979273635928}\) & \(\num{282479.6} \pm \num{4200.325969288081}\) & \(\num{1664.5666666666666} \pm \num{68.81643916137027}\) & \(\num{44549.433333333334} \pm \num{1469.6071650411309}\) & \(\num{3307.0} \pm \num{2163.1080926966306}\) \\
\texttt{pdir.format} & \(\num{392.8666666666667} \pm \num{285.68559199102845}\) & \(\num{19428.9} \pm \num{15639.08928327813}\) & \(\num{409.03333333333336} \pm \num{315.39274731272957}\) & \(\num{1775.9333333333334} \pm \num{69.8915087010271}\) & \(\num{387.2} \pm \num{292.5124695249524}\) \\
 & \(\num{2031.3333333333333} \pm \num{1496.5905005835034}\) & \(\num{595765.7666666667} \pm \num{68832.61990218627}\) & \(\num{2562.5333333333333} \pm \num{1376.724667170383}\) & \(\num{3893.233333333333} \pm \num{370.5805960394035}\) & \(\num{2919.8} \pm \num{1583.5851598890063}\) \\
\rowcolor{gray!25}
\texttt{py\_backwards.conf} & \(\num{8823.966666666667} \pm \num{1101.6421436399744}\) & \(\num{1011694.1333333333} \pm \num{14098.16284615771}\) & \(\num{8997.866666666667} \pm \num{1103.456660815843}\) & \(\num{1900.5} \pm \num{68.4859663449885}\) & \(\num{2439.4} \pm \num{1166.8984117943926}\) \\
\rowcolor{gray!25}
 & \(\num{7627.633333333333} \pm \num{704.4725335843212}\) & \(\num{985060.3} \pm \num{15586.725676699696}\) & \(\num{7624.833333333333} \pm \num{684.2424496368648}\) & \(\num{1530.3666666666666} \pm \num{30.86956243709119}\) & \(\num{3536.5} \pm \num{2287.8139807127736}\) \\
\texttt{py\_backwards.files} & \(\num{7204.1} \pm \num{107.62910451142402}\) & \(\num{711448.0} \pm \num{19188.538852928454}\) & \(\num{3132.3} \pm \num{42.47120728535819}\) & \(\num{1475.5} \pm \num{31.422318007516843}\) & \(\num{4494.566666666667} \pm \num{3876.2129108041854}\) \\
 & \(\num{1078.5} \pm \num{440.91462540558996}\) & \(\num{481801.93333333335} \pm \num{41562.78766822581}\) & \(\num{989.6333333333333} \pm \num{467.0460719600726}\) & \(\num{1494.9333333333334} \pm \num{31.756545166619432}\) & \(\num{1457.3} \pm \num{1137.7193202737387}\) \\
\rowcolor{gray!25}
\texttt{py\_backwards.transformers.base} & \(\num{5213.9} \pm \num{737.0058882467255}\) & \(\num{375226.0333333333} \pm \num{5719.50405664888}\) & \(\num{4720.7} \pm \num{592.2459967696321}\) & \(\num{2016.3} \pm \num{57.24849041828451}\) & \(\num{1886.5333333333333} \pm \num{678.6869540584933}\) \\
\rowcolor{gray!25}
 & \(\num{2619.3333333333335} \pm \num{290.52679066129855}\) & \(\num{462766.93333333335} \pm \num{17730.08188310503}\) & \(\num{1764.5} \pm \num{21.52744839693638}\) & \(\num{2086.5333333333333} \pm \num{58.72656294558961}\) & \(\num{4779.366666666667} \pm \num{3380.135046101717}\) \\
\texttt{py\_backwards.transformers.class\_without\_bases} & \(\num{11.166666666666666} \pm \num{16.062557303444454}\) & \(\num{187.76666666666668} \pm \num{153.37033911268577}\) & \(\num{11.166666666666666} \pm \num{16.062557303444454}\) & \(\num{447.53333333333336} \pm \num{515.1165742406969}\) & \(\num{0.36666666666666664} \pm \num{1.4735210781716332}\) \\
 & \(\num{10353.766666666666} \pm \num{1657.806146550383}\) & \(\num{641665.6333333333} \pm \num{187633.75853094007}\) & \(\num{10210.033333333333} \pm \num{1600.8845934698713}\) & \(\num{2110.5666666666666} \pm \num{41.66672643673874}\) & \(\num{4914.8} \pm \num{4030.6117393149457}\) \\
\rowcolor{gray!25}
\texttt{py\_backwards.transformers.dict\_unpacking} & \(\num{4864.066666666667} \pm \num{1611.8269979325846}\) & \(\num{393356.8} \pm \num{42076.77471529132}\) & \(\num{4517.5} \pm \num{1362.4009676125909}\) & \(\num{2448.8333333333335} \pm \num{91.19591768439447}\) & \(\num{2360.9333333333334} \pm \num{1108.6145418038004}\) \\
\rowcolor{gray!25}
 & \(\num{3549.3} \pm \num{54.055622693921364}\) & \(\num{477760.5333333333} \pm \num{7637.11477716161}\) & \(\num{2524.9666666666667} \pm \num{32.74613252587699}\) & \(\num{2500.733333333333} \pm \num{82.0415930397853}\) & \(\num{3338.366666666667} \pm \num{2529.538658814445}\) \\
\texttt{py\_backwards.transformers.formatted\_values} & \(\num{38.766666666666666} \pm \num{38.90632723414759}\) & \(\num{1106.5} \pm \num{1858.461372322221}\) & \(\num{38.766666666666666} \pm \num{38.90632723414759}\) & \(\num{1171.4} \pm \num{831.534418803679}\) & \(\num{16.733333333333334} \pm \num{21.492473956750747}\) \\
 & \(\num{10525.0} \pm \num{965.4618691018591}\) & \(\num{616379.0666666667} \pm \num{130006.33029837653}\) & \(\num{10418.166666666666} \pm \num{950.0051209783331}\) & \(\num{2507.733333333333} \pm \num{76.52402522594855}\) & \(\num{3711.5666666666666} \pm \num{2396.0249075231386}\) \\
\rowcolor{gray!25}
\texttt{py\_backwards.transformers.functions\_annotations} & \(\num{0.0} \pm \num{0.0}\) & \(\num{3.566666666666667} \pm \num{3.0021065401082825}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{5.066666666666666} \pm \num{2.1803722132942687}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{8.566666666666666} \pm \num{6.871647562985537}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{9.366666666666667} \pm \num{5.851515178571912}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{py\_backwards.transformers.import\_pathlib} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{py\_backwards.transformers.metaclass} & \(\num{7565.4} \pm \num{963.5028980147172}\) & \(\num{532059.8} \pm \num{11306.948911300458}\) & \(\num{7693.033333333334} \pm \num{945.8446501930698}\) & \(\num{2413.8333333333335} \pm \num{142.82617439375048}\) & \(\num{1943.0} \pm \num{622.6872796804686}\) \\
\rowcolor{gray!25}
 & \(\num{8323.833333333334} \pm \num{753.4975955082947}\) & \(\num{610800.1} \pm \num{14325.251176350006}\) & \(\num{8297.766666666666} \pm \num{631.241179294239}\) & \(\num{2516.1} \pm \num{77.73090185665077}\) & \(\num{3686.5333333333333} \pm \num{2786.365668174515}\) \\
\texttt{py\_backwards.transformers.python2\_future} & \(\num{9126.1} \pm \num{349.83930793910275}\) & \(\num{601276.6333333333} \pm \num{12032.880577769007}\) & \(\num{9230.133333333333} \pm \num{294.35431773258586}\) & \(\num{2049.5666666666666} \pm \num{53.927590873979014}\) & \(\num{3375.7} \pm \num{2164.6577040867382}\) \\
 & \(\num{12165.733333333334} \pm \num{288.64068264567436}\) & \(\num{618195.2666666667} \pm \num{9184.463552871393}\) & \(\num{12081.433333333332} \pm \num{482.5510288065904}\) & \(\num{2076.9666666666667} \pm \num{58.04307754224195}\) & \(\num{3849.8333333333335} \pm \num{2334.5799752674016}\) \\
\rowcolor{gray!25}
\texttt{py\_backwards.transformers.return\_from\_generator} & \(\num{4743.633333333333} \pm \num{318.2808869355899}\) & \(\num{272045.13333333336} \pm \num{17913.92724945735}\) & \(\num{3660.5} \pm \num{446.5637962687202}\) & \(\num{2010.0666666666666} \pm \num{98.86177509387863}\) & \(\num{2213.9666666666667} \pm \num{1228.6140631182577}\) \\
\rowcolor{gray!25}
 & \(\num{4431.0} \pm \num{683.7508620684221}\) & \(\num{430778.1666666667} \pm \num{40072.345878581196}\) & \(\num{2677.4333333333334} \pm \num{1026.4929474986022}\) & \(\num{2069.8} \pm \num{52.17834139127869}\) & \(\num{4991.9} \pm \num{3593.4544550737883}\) \\
\texttt{py\_backwards.transformers.starred\_unpacking} & \(\num{4949.566666666667} \pm \num{1158.304399374014}\) & \(\num{416923.6} \pm \num{43064.77783813909}\) & \(\num{3967.0} \pm \num{955.9089193374888}\) & \(\num{2412.733333333333} \pm \num{115.57291573104277}\) & \(\num{2298.3} \pm \num{1343.6049591330393}\) \\
 & \(\num{4548.833333333333} \pm \num{980.9821638272158}\) & \(\num{510448.3} \pm \num{21947.298454675936}\) & \(\num{2790.8} \pm \num{851.6140618524495}\) & \(\num{2525.3333333333335} \pm \num{62.87992571140065}\) & \(\num{5300.433333333333} \pm \num{3775.880501865468}\) \\
\rowcolor{gray!25}
\texttt{py\_backwards.transformers.string\_types} & \(\num{10452.233333333334} \pm \num{646.8706998302292}\) & \(\num{986315.0666666667} \pm \num{11238.004639225968}\) & \(\num{9168.566666666668} \pm \num{417.2459527155072}\) & \(\num{1515.2} \pm \num{73.416337559767}\) & \(\num{4645.6} \pm \num{4217.932256940352}\) \\
\rowcolor{gray!25}
 & \(\num{6144.6} \pm \num{327.1846046458198}\) & \(\num{1038793.0666666667} \pm \num{10457.906795679834}\) & \(\num{5216.266666666666} \pm \num{275.80201961368687}\) & \(\num{5822.533333333334} \pm \num{3418.797466879287}\) & \(\num{5688.133333333333} \pm \num{4878.852781583782}\) \\
\texttt{py\_backwards.transformers.variables\_annotations} & \(\num{10495.7} \pm \num{453.31097265677846}\) & \(\num{953920.1666666666} \pm \num{14535.553802678958}\) & \(\num{8118.3} \pm \num{356.6843625430734}\) & \(\num{1513.6666666666667} \pm \num{84.77570135498665}\) & \(\num{4573.433333333333} \pm \num{4143.062274772572}\) \\
 & \(\num{6171.9} \pm \num{356.02056798391044}\) & \(\num{1005149.6333333333} \pm \num{13382.1696670925}\) & \(\num{4544.866666666667} \pm \num{195.7277724788698}\) & \(\num{6780.933333333333} \pm \num{3763.9564193062574}\) & \(\num{5582.733333333334} \pm \num{5074.53897979622}\) \\
\rowcolor{gray!25}
\texttt{py\_backwards.transformers.yield\_from} & \(\num{6265.233333333334} \pm \num{939.7758604135839}\) & \(\num{369913.6666666667} \pm \num{16495.672917116954}\) & \(\num{5684.066666666667} \pm \num{889.700760749456}\) & \(\num{1401.9333333333334} \pm \num{42.84449293331225}\) & \(\num{2132.3} \pm \num{1013.0351850784339}\) \\
\rowcolor{gray!25}
 & \(\num{6868.3} \pm \num{739.5155054213676}\) & \(\num{463601.1666666667} \pm \num{19774.137442426007}\) & \(\num{5203.6} \pm \num{830.548119804232}\) & \(\num{1759.2666666666667} \pm \num{68.192391795937}\) & \(\num{3411.9333333333334} \pm \num{1837.059493214413}\) \\
\texttt{py\_backwards.types} & \(\num{10300.466666666667} \pm \num{449.20571536061703}\) & \(\num{922807.9333333333} \pm \num{27869.805914637087}\) & \(\num{10408.566666666668} \pm \num{455.20466661244484}\) & \(\num{4518.5} \pm \num{353.97094659658546}\) & \(\num{4978.866666666667} \pm \num{4399.038254870727}\) \\
 & \(\num{6378.433333333333} \pm \num{417.72946890948725}\) & \(\num{990758.2333333333} \pm \num{24110.99727865408}\) & \(\num{6314.4} \pm \num{387.8771223840941}\) & \(\num{7361.9} \pm \num{2614.5722449643517}\) & \(\num{5993.933333333333} \pm \num{5468.923634458633}\) \\
\rowcolor{gray!25}
\texttt{py\_backwards.utils.helpers} & \(\num{8358.433333333332} \pm \num{840.9594964756886}\) & \(\num{650601.9666666667} \pm \num{19357.52445786345}\) & \(\num{8461.166666666666} \pm \num{872.3760294629886}\) & \(\num{1722.0666666666666} \pm \num{48.889695221494016}\) & \(\num{2427.633333333333} \pm \num{1233.9463880192475}\) \\
\rowcolor{gray!25}
 & \(\num{8640.566666666668} \pm \num{804.7695186579319}\) & \(\num{641157.9} \pm \num{14847.140496428583}\) & \(\num{8638.466666666667} \pm \num{786.7399663882874}\) & \(\num{1723.2333333333333} \pm \num{43.606139502355056}\) & \(\num{2345.2} \pm \num{844.7455605500188}\) \\
\texttt{py\_backwards.utils.snippet} & \(\num{3969.6666666666665} \pm \num{679.8114004853737}\) & \(\num{181809.6} \pm \num{8007.415091973964}\) & \(\num{3510.9333333333334} \pm \num{522.9938968018213}\) & \(\num{1555.7333333333333} \pm \num{48.66063574661113}\) & \(\num{841.7} \pm \num{196.61482562404194}\) \\
 & \(\num{4150.766666666666} \pm \num{1070.1864060424991}\) & \(\num{289672.2} \pm \num{4322.409963163509}\) & \(\num{3204.6} \pm \num{711.4224992322025}\) & \(\num{2654.366666666667} \pm \num{99.23864769031418}\) & \(\num{885.5333333333333} \pm \num{173.8435153121679}\) \\
\rowcolor{gray!25}
\texttt{pymonet.box} & \(\num{2.0} \pm \num{2.084425001338954}\) & \(\num{161.86666666666667} \pm \num{123.44082299470138}\) & \(\num{2.0} \pm \num{2.084425001338954}\) & \(\num{344.8333333333333} \pm \num{234.18782372619035}\) & \(\num{3.1666666666666665} \pm \num{3.851406669430448}\) \\
\rowcolor{gray!25}
 & \(\num{0.9} \pm \num{1.5165750888103104}\) & \(\num{105.96666666666667} \pm \num{59.47731142807856}\) & \(\num{0.9} \pm \num{1.5165750888103102}\) & \(\num{176.56666666666666} \pm \num{155.01361082250128}\) & \(\num{2.1} \pm \num{1.5833182092441616}\) \\
\texttt{pymonet.immutable\_list} & \(\num{3040.3333333333335} \pm \num{1268.7192383451613}\) & \(\num{307721.5333333333} \pm \num{3934.821441274387}\) & \(\num{3122.3333333333335} \pm \num{973.8945398310044}\) & \(\num{1662.6} \pm \num{63.45598528874576}\) & \(\num{808.6666666666666} \pm \num{128.66565421553898}\) \\
 & \(\num{4318.733333333334} \pm \num{1015.7238945131977}\) & \(\num{310338.76666666666} \pm \num{3697.0794035416598}\) & \(\num{4606.4} \pm \num{1139.0374218066156}\) & \(\num{1777.0} \pm \num{68.31923039217664}\) & \(\num{880.3333333333334} \pm \num{171.2236555791432}\) \\
\rowcolor{gray!25}
\texttt{pymonet.lazy} & \(\num{6671.1} \pm \num{1867.8946907848067}\) & \(\num{390494.1} \pm \num{8662.747005385205}\) & \(\num{6688.233333333334} \pm \num{1856.0258560054922}\) & \(\num{1781.5333333333333} \pm \num{57.772283853152246}\) & \(\num{1594.1666666666667} \pm \num{410.3198149915656}\) \\
\rowcolor{gray!25}
 & \(\num{6747.033333333334} \pm \num{1543.0304594694735}\) & \(\num{389420.73333333334} \pm \num{8574.109033569624}\) & \(\num{6615.166666666667} \pm \num{1373.044592874896}\) & \(\num{1846.6333333333334} \pm \num{57.10696758825876}\) & \(\num{1374.7} \pm \num{371.76347226475167}\) \\
\texttt{pymonet.maybe} & \(\num{2706.266666666667} \pm \num{542.4799969827798}\) & \(\num{293936.8} \pm \num{5141.4281217415155}\) & \(\num{3088.1} \pm \num{1001.5051207540337}\) & \(\num{1507.6} \pm \num{59.33807290898251}\) & \(\num{979.5333333333333} \pm \num{167.82764831883298}\) \\
 & \(\num{3945.5666666666666} \pm \num{1255.803841571504}\) & \(\num{300044.5333333333} \pm \num{5956.4536529331135}\) & \(\num{3919.1} \pm \num{1174.5445881937271}\) & \(\num{1485.5666666666666} \pm \num{44.50701868968172}\) & \(\num{965.2666666666667} \pm \num{159.47520255477042}\) \\
\rowcolor{gray!25}
\texttt{pymonet.monad\_try} & \(\num{4370.966666666666} \pm \num{1240.4200479685499}\) & \(\num{400907.93333333335} \pm \num{5551.6706024548075}\) & \(\num{4578.966666666666} \pm \num{1182.940039385602}\) & \(\num{1526.0666666666666} \pm \num{59.97466898233145}\) & \(\num{1190.0} \pm \num{218.91109831508598}\) \\
\rowcolor{gray!25}
 & \(\num{5234.266666666666} \pm \num{1042.1065513505882}\) & \(\num{394689.76666666666} \pm \num{4856.600795670337}\) & \(\num{5185.0} \pm \num{1230.9639340356612}\) & \(\num{1716.1333333333334} \pm \num{102.72451721367013}\) & \(\num{1313.3} \pm \num{260.6570146962188}\) \\
\texttt{pymonet.semigroups} & \(\num{9141.866666666667} \pm \num{1439.404683776651}\) & \(\num{318639.9666666667} \pm \num{4594.554051252968}\) & \(\num{9207.566666666668} \pm \num{1388.132799056377}\) & \(\num{1529.0333333333333} \pm \num{57.82284677526179}\) & \(\num{947.5333333333333} \pm \num{177.82493004954742}\) \\
 & \(\num{10081.033333333333} \pm \num{1455.178208859736}\) & \(\num{318025.0333333333} \pm \num{3664.686094505827}\) & \(\num{10011.9} \pm \num{1435.8801301904912}\) & \(\num{1594.6333333333334} \pm \num{34.8647468757862}\) & \(\num{934.0333333333333} \pm \num{176.54548760985736}\) \\
\rowcolor{gray!25}
\texttt{pymonet.task} & \(\num{4709.766666666666} \pm \num{58.60721582814215}\) & \(\num{645592.5333333333} \pm \num{18723.016369741526}\) & \(\num{4737.766666666666} \pm \num{59.55390680796646}\) & \(\num{1355.9} \pm \num{35.29515938286819}\) & \(\num{3960.866666666667} \pm \num{3188.887112472305}\) \\
\rowcolor{gray!25}
 & \(\num{4720.233333333334} \pm \num{78.87907958009082}\) & \(\num{631855.4333333333} \pm \num{24101.327926905396}\) & \(\num{4729.633333333333} \pm \num{85.7785775576635}\) & \(\num{1346.2} \pm \num{38.185933499672096}\) & \(\num{4012.766666666667} \pm \num{3255.946927078822}\) \\
\texttt{pymonet.validation} & \(\num{9336.6} \pm \num{636.7750428309937}\) & \(\num{388038.86666666664} \pm \num{5424.976750201782}\) & \(\num{9438.9} \pm \num{678.1705791928448}\) & \(\num{1874.7} \pm \num{83.14057476595765}\) & \(\num{1268.6} \pm \num{234.95422885143483}\) \\
 & \(\num{9200.133333333333} \pm \num{785.8619574021598}\) & \(\num{387787.9666666667} \pm \num{6207.020977300115}\) & \(\num{9230.766666666666} \pm \num{641.1203385525585}\) & \(\num{1851.2333333333333} \pm \num{92.32875419160985}\) & \(\num{1212.4666666666667} \pm \num{261.6885136205247}\) \\
\rowcolor{gray!25}
\texttt{pypara.accounting.generic} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.2333333333333334} \pm \num{0.5683207771559354}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{pypara.accounting.journaling} & \(\num{3703.3333333333335} \pm \num{167.35989165069788}\) & \(\num{375703.86666666664} \pm \num{8445.607745361238}\) & \(\num{2759.9} \pm \num{181.92710741885912}\) & \(\num{2024.0666666666666} \pm \num{128.714850128795}\) & \(\num{3698.5} \pm \num{2005.5961148401911}\) \\
 & \(\num{4037.133333333333} \pm \num{124.64480108204117}\) & \(\num{438729.63333333336} \pm \num{9571.636859558785}\) & \(\num{2958.9333333333334} \pm \num{93.57347595498871}\) & \(\num{1920.6333333333334} \pm \num{40.79256468197769}\) & \(\num{2671.9} \pm \num{1302.65522868777}\) \\
\rowcolor{gray!25}
\texttt{pypara.commons.errors} & \(\num{10443.066666666668} \pm \num{581.898375612297}\) & \(\num{1003053.0333333333} \pm \num{11166.725348053053}\) & \(\num{9128.4} \pm \num{412.0354521071013}\) & \(\num{1425.1666666666667} \pm \num{55.672740394096884}\) & \(\num{4402.066666666667} \pm \num{4146.9681981878775}\) \\
\rowcolor{gray!25}
 & \(\num{7974.8} \pm \num{455.50558496140803}\) & \(\num{1074325.1333333333} \pm \num{11984.300913920773}\) & \(\num{6689.1} \pm \num{350.5034162851857}\) & \(\num{1954.6} \pm \num{100.3654013746941}\) & \(\num{5328.233333333334} \pm \num{5336.620341359885}\) \\
\texttt{pypara.commons.numbers} & \(\num{0.0} \pm \num{0.0}\) & \(\num{11.733333333333333} \pm \num{14.241593608362342}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{20.8} \pm \num{31.457031449045015}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{17.533333333333335} \pm \num{12.864635656508607}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{20.833333333333332} \pm \num{26.526607765416024}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{pypara.commons.others} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.1333333333333333} \pm \num{0.43417248545530474}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{3.2} \pm \num{1.9369367924460092}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.1666666666666667} \pm \num{0.5920934999167601}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{2.966666666666667} \pm \num{1.6291172420994586}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{pypara.commons.zeitgeist} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{pypara.monetary} & \(\num{1110.0333333333333} \pm \num{258.6441415420481}\) & \(\num{67471.2} \pm \num{1965.0971266686488}\) & \(\num{1105.2} \pm \num{343.0269316862292}\) & \(\num{1859.5666666666666} \pm \num{126.98375767256094}\) & \(\num{385.1333333333333} \pm \num{31.02472132563536}\) \\
\rowcolor{gray!25}
 & \(\num{999.2666666666667} \pm \num{421.70008408766085}\) & \(\num{82161.0} \pm \num{2416.902235050707}\) & \(\num{667.7666666666667} \pm \num{401.1648283938036}\) & \(\num{1782.0333333333333} \pm \num{180.63785133059275}\) & \(\num{369.26666666666665} \pm \num{27.317965963223106}\) \\
\texttt{pytutils.debug} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0666666666666667} \pm \num{0.2537081317024625}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.5} \pm \num{1.137147065368355}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{pytutils.excs} & \(\num{9209.8} \pm \num{714.5703990317636}\) & \(\num{1123072.1666666667} \pm \num{17324.594441356232}\) & \(\num{7876.6} \pm \num{526.9714119053492}\) & \(\num{1597.4333333333334} \pm \num{56.557985706056016}\) & \(\num{5342.0} \pm \num{5128.813380271812}\) \\
\rowcolor{gray!25}
 & \(\num{7833.8} \pm \num{465.7982691962336}\) & \(\num{1142563.5333333334} \pm \num{21857.5557073258}\) & \(\num{6527.333333333333} \pm \num{372.44340771991523}\) & \(\num{1645.1666666666667} \pm \num{53.80493717464798}\) & \(\num{5532.6} \pm \num{5751.672569933387}\) \\
\texttt{pytutils.files} & \(\num{5559.833333333333} \pm \num{289.9783681983684}\) & \(\num{359053.7} \pm \num{8295.090567774785}\) & \(\num{3844.3} \pm \num{261.13388691732774}\) & \(\num{1991.6666666666667} \pm \num{45.687343250985094}\) & \(\num{2061.2} \pm \num{796.2232575490804}\) \\
 & \(\num{5579.6} \pm \num{306.75741286043535}\) & \(\num{361615.3333333333} \pm \num{9094.763875660708}\) & \(\num{3843.8333333333335} \pm \num{294.75461253251905}\) & \(\num{1976.7} \pm \num{50.47713719408367}\) & \(\num{2143.3333333333335} \pm \num{834.2773595415844}\) \\
\rowcolor{gray!25}
\texttt{pytutils.lazy.lazy\_import} & \(\num{3944.5666666666666} \pm \num{164.13675612928287}\) & \(\num{206301.53333333333} \pm \num{4954.707143531384}\) & \(\num{2793.133333333333} \pm \num{215.2334311510586}\) & \(\num{2247.366666666667} \pm \num{81.63775467579781}\) & \(\num{914.9666666666667} \pm \num{185.28160921322896}\) \\
\rowcolor{gray!25}
 & \(\num{3930.5333333333333} \pm \num{229.8697882285314}\) & \(\num{204984.9} \pm \num{6267.206688733852}\) & \(\num{2722.5333333333333} \pm \num{179.61889412430082}\) & \(\num{2249.6} \pm \num{84.32596851218041}\) & \(\num{973.2} \pm \num{246.24397769635735}\) \\
\texttt{pytutils.meth} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0333333333333334} \pm \num{0.18257418583505533}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0666666666666667} \pm \num{0.2537081317024625}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0333333333333334} \pm \num{0.18257418583505533}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0666666666666667} \pm \num{0.2537081317024624}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{pytutils.path} & \(\num{11594.7} \pm \num{140.25153511975645}\) & \(\num{909525.3666666667} \pm \num{24657.830051748668}\) & \(\num{11633.566666666668} \pm \num{149.34654985644292}\) & \(\num{1454.7} \pm \num{35.85425478526777}\) & \(\num{4148.866666666667} \pm \num{3827.6694785184372}\) \\
\rowcolor{gray!25}
 & \(\num{11607.166666666666} \pm \num{103.2369498585267}\) & \(\num{912704.6333333333} \pm \num{26262.4718923296}\) & \(\num{11590.4} \pm \num{170.7768457212006}\) & \(\num{1444.8} \pm \num{30.97429412515682}\) & \(\num{4255.2} \pm \num{3752.057875812722}\) \\
\texttt{pytutils.pretty} & \(\num{2904.6} \pm \num{645.0998639612}\) & \(\num{231645.13333333333} \pm \num{7588.952409342436}\) & \(\num{2572.733333333333} \pm \num{544.1495695330361}\) & \(\num{1949.3666666666666} \pm \num{72.60876898373455}\) & \(\num{1464.2} \pm \num{329.42137359210676}\) \\
 & \(\num{2482.1} \pm \num{335.4841432092247}\) & \(\num{257712.2} \pm \num{5575.842916948321}\) & \(\num{2233.4666666666667} \pm \num{321.45195740505335}\) & \(\num{1957.6333333333334} \pm \num{60.2302955807717}\) & \(\num{1684.9} \pm \num{498.8986041686019}\) \\
\rowcolor{gray!25}
\texttt{pytutils.props} & \(\num{8306.466666666667} \pm \num{116.37150182403599}\) & \(\num{574034.6333333333} \pm \num{9881.03753271834}\) & \(\num{8304.866666666667} \pm \num{107.01618741020488}\) & \(\num{2002.7} \pm \num{63.00035577348914}\) & \(\num{1887.7} \pm \num{602.4596795780124}\) \\
\rowcolor{gray!25}
 & \(\num{8256.366666666667} \pm \num{111.60103921569453}\) & \(\num{570676.3666666667} \pm \num{9401.236934329563}\) & \(\num{8288.333333333334} \pm \num{118.3686041008409}\) & \(\num{1974.1666666666667} \pm \num{51.83467308022048}\) & \(\num{1957.5} \pm \num{682.2156474716571}\) \\
\texttt{pytutils.python} & \(\num{9991.6} \pm \num{497.43303829380574}\) & \(\num{834850.3} \pm \num{9848.022644690906}\) & \(\num{7618.7} \pm \num{325.2726336581308}\) & \(\num{1468.9333333333334} \pm \num{68.33887838449337}\) & \(\num{4074.3333333333335} \pm \num{2541.3669595295573}\) \\
 & \(\num{7610.033333333334} \pm \num{428.9194509488919}\) & \(\num{878590.9666666667} \pm \num{12989.269564776796}\) & \(\num{5514.0} \pm \num{263.3793645204051}\) & \(\num{2380.866666666667} \pm \num{583.704385108937}\) & \(\num{4608.666666666667} \pm \num{3141.170584937749}\) \\
\rowcolor{gray!25}
\texttt{pytutils.pythree} & \(\num{0.2} \pm \num{0.8051557998728973}\) & \(\num{49.666666666666664} \pm \num{40.115637447460465}\) & \(\num{0.2} \pm \num{0.8051557998728973}\) & \(\num{32.833333333333336} \pm \num{32.25660406408471}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.2} \pm \num{0.8051557998728974}\) & \(\num{49.666666666666664} \pm \num{40.115637447460465}\) & \(\num{0.2} \pm \num{0.8051557998728974}\) & \(\num{32.833333333333336} \pm \num{32.256604064084705}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{pytutils.rand} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0333333333333334} \pm \num{0.1825741858350553}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0333333333333334} \pm \num{0.1825741858350553}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{sanic.base} & \(\num{6946.9} \pm \num{364.15375210536246}\) & \(\num{725980.7} \pm \num{24058.44813287152}\) & \(\num{6970.266666666666} \pm \num{384.18457609038273}\) & \(\num{13416.866666666667} \pm \num{171.16915072792625}\) & \(\num{4206.433333333333} \pm \num{3010.2876100801896}\) \\
\rowcolor{gray!25}
 & \(\num{5874.5} \pm \num{380.3511762061205}\) & \(\num{771802.9666666667} \pm \num{19757.20216909709}\) & \(\num{5824.233333333334} \pm \num{376.58169268349707}\) & \(\num{14858.9} \pm \num{204.07425119304003}\) & \(\num{4475.933333333333} \pm \num{3407.662166893626}\) \\
\texttt{sanic.config} & \(\num{5738.166666666667} \pm \num{1248.8944375294311}\) & \(\num{316858.7} \pm \num{4848.679579588369}\) & \(\num{5795.566666666667} \pm \num{1115.309379788262}\) & \(\num{2193.266666666667} \pm \num{69.97828891549314}\) & \(\num{1357.3666666666666} \pm \num{280.017177223523}\) \\
 & \(\num{6349.9} \pm \num{1605.1807578952726}\) & \(\num{319905.9666666667} \pm \num{4738.050548363806}\) & \(\num{6073.433333333333} \pm \num{1662.4229862034126}\) & \(\num{2195.133333333333} \pm \num{73.99241961795505}\) & \(\num{1494.6333333333334} \pm \num{398.4952284864108}\) \\
\rowcolor{gray!25}
\texttt{sanic.cookies} & \(\num{5322.8} \pm \num{1424.455549953421}\) & \(\num{279201.1666666667} \pm \num{4578.509764204892}\) & \(\num{3643.7} \pm \num{850.5217526460672}\) & \(\num{3203.2} \pm \num{332.4463555377692}\) & \(\num{1365.5} \pm \num{441.874436057778}\) \\
\rowcolor{gray!25}
 & \(\num{4787.266666666666} \pm \num{1304.0728754052882}\) & \(\num{283750.2} \pm \num{14722.932959303249}\) & \(\num{3198.133333333333} \pm \num{685.3844998565974}\) & \(\num{3205.6} \pm \num{376.5647446277356}\) & \(\num{1418.9333333333334} \pm \num{388.3182957968562}\) \\
\texttt{sanic.handlers} & \(\num{4658.333333333333} \pm \num{813.3203692202142}\) & \(\num{341866.1666666667} \pm \num{5527.377678949316}\) & \(\num{3258.3333333333335} \pm \num{480.74908024968653}\) & \(\num{1986.6666666666667} \pm \num{62.95117611858132}\) & \(\num{1799.2} \pm \num{572.4754113075287}\) \\
 & \(\num{4837.566666666667} \pm \num{951.4410733681589}\) & \(\num{344025.0333333333} \pm \num{5099.702820843538}\) & \(\num{3370.3} \pm \num{598.7929899619619}\) & \(\num{1988.0333333333333} \pm \num{60.51758555097469}\) & \(\num{1961.3} \pm \num{757.4790380620763}\) \\
\rowcolor{gray!25}
\texttt{sanic.headers} & \(\num{4315.266666666666} \pm \num{781.2775096765788}\) & \(\num{248375.6} \pm \num{5894.561120219214}\) & \(\num{2616.4333333333334} \pm \num{494.3808864828213}\) & \(\num{2197.5333333333333} \pm \num{52.5939116270114}\) & \(\num{1336.1333333333334} \pm \num{411.31393609138564}\) \\
\rowcolor{gray!25}
 & \(\num{5458.4} \pm \num{916.8668011409742}\) & \(\num{273285.76666666666} \pm \num{5477.90859086614}\) & \(\num{2809.8} \pm \num{480.6720439063452}\) & \(\num{2902.6666666666665} \pm \num{295.95401941719837}\) & \(\num{1341.9333333333334} \pm \num{450.8964965207788}\) \\
\texttt{sanic.helpers} & \(\num{11851.6} \pm \num{2101.9482522584644}\) & \(\num{483738.36666666664} \pm \num{28236.193821947298}\) & \(\num{11797.733333333334} \pm \num{1427.1663492759865}\) & \(\num{2796.7} \pm \num{99.38019992901522}\) & \(\num{1917.9333333333334} \pm \num{659.0300570474415}\) \\
 & \(\num{11863.1} \pm \num{2047.416376129042}\) & \(\num{473788.56666666665} \pm \num{34751.592793745425}\) & \(\num{11548.666666666666} \pm \num{1389.1695195414375}\) & \(\num{2781.5333333333333} \pm \num{99.44457244367713}\) & \(\num{2014.9} \pm \num{712.7537829941093}\) \\
\rowcolor{gray!25}
\texttt{sanic.mixins.listeners} & \(\num{18.8} \pm \num{21.52208168370337}\) & \(\num{1228.5} \pm \num{1559.320160220141}\) & \(\num{18.8} \pm \num{21.522081683703373}\) & \(\num{369.0} \pm \num{436.1674781153648}\) & \(\num{21.833333333333332} \pm \num{26.221974640041676}\) \\
\rowcolor{gray!25}
 & \(\num{232.6} \pm \num{409.69472234487154}\) & \(\num{14878.8} \pm \num{16922.213698017742}\) & \(\num{232.6} \pm \num{409.6947223448715}\) & \(\num{1202.0333333333333} \pm \num{796.8186953964705}\) & \(\num{269.2} \pm \num{332.4985247569035}\) \\
\texttt{sanic.mixins.middleware} & \(\num{73.5} \pm \num{105.25003071504179}\) & \(\num{1804.4333333333334} \pm \num{1696.1059393420164}\) & \(\num{73.5} \pm \num{105.25003071504179}\) & \(\num{940.1666666666666} \pm \num{644.4630528096872}\) & \(\num{65.7} \pm \num{66.13004429622507}\) \\
 & \(\num{139.36666666666667} \pm \num{165.38387598790158}\) & \(\num{7289.033333333334} \pm \num{9656.606387851018}\) & \(\num{139.36666666666667} \pm \num{165.38387598790158}\) & \(\num{880.0} \pm \num{675.648960068303}\) & \(\num{178.53333333333333} \pm \num{210.78093438176657}\) \\
\rowcolor{gray!25}
\texttt{sanic.mixins.routes} & \(\num{3183.9666666666667} \pm \num{837.3924834057013}\) & \(\num{109221.73333333334} \pm \num{2595.1979518324615}\) & \(\num{1976.0666666666666} \pm \num{344.8179863031523}\) & \(\num{2340.3} \pm \num{65.4107183033906}\) & \(\num{557.0666666666667} \pm \num{62.51396165896743}\) \\
\rowcolor{gray!25}
 & \(\num{4594.2} \pm \num{881.9002758542057}\) & \(\num{143310.96666666667} \pm \num{3829.9953496265393}\) & \(\num{2621.633333333333} \pm \num{484.34395610567077}\) & \(\num{3743.4333333333334} \pm \num{303.5362482850912}\) & \(\num{667.1} \pm \num{156.34893557415867}\) \\
\texttt{sanic.mixins.signals} & \(\num{9915.0} \pm \num{630.575817859332}\) & \(\num{580175.0} \pm \num{8383.334239162676}\) & \(\num{10041.366666666667} \pm \num{690.4583426887576}\) & \(\num{1849.0} \pm \num{78.065401405179}\) & \(\num{1936.2333333333333} \pm \num{707.2781574133496}\) \\
 & \(\num{7825.833333333333} \pm \num{1499.819738210708}\) & \(\num{608599.0333333333} \pm \num{10310.922148410136}\) & \(\num{7655.933333333333} \pm \num{1402.8998768150975}\) & \(\num{2044.9333333333334} \pm \num{52.917589366559554}\) & \(\num{2003.3333333333333} \pm \num{410.86438179755265}\) \\
\rowcolor{gray!25}
\texttt{sanic.models.futures} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{sanic.models.protocol\_types} & \(\num{6084.066666666667} \pm \num{216.80261694140984}\) & \(\num{730604.3666666667} \pm \num{20788.611702470465}\) & \(\num{6108.466666666666} \pm \num{206.88606448516762}\) & \(\num{14314.833333333334} \pm \num{192.65604214431647}\) & \(\num{5421.233333333334} \pm \num{4764.735913247292}\) \\
 & \(\num{4536.966666666666} \pm \num{235.44242774319414}\) & \(\num{771547.4} \pm \num{17576.83786554692}\) & \(\num{4532.333333333333} \pm \num{246.1847264560291}\) & \(\num{14460.166666666666} \pm \num{169.88882436369428}\) & \(\num{6556.433333333333} \pm \num{5738.279188670279}\) \\
\rowcolor{gray!25}
\texttt{sanic.views} & \(\num{8700.066666666668} \pm \num{1640.497862473953}\) & \(\num{509152.06666666665} \pm \num{11450.782767802484}\) & \(\num{7321.366666666667} \pm \num{1083.6315852925652}\) & \(\num{2199.6} \pm \num{71.28263318020349}\) & \(\num{1480.5333333333333} \pm \num{364.52933596846384}\) \\
\rowcolor{gray!25}
 & \(\num{8602.0} \pm \num{1353.981612466193}\) & \(\num{525752.3333333334} \pm \num{11115.260656919583}\) & \(\num{7266.0} \pm \num{925.535557915263}\) & \(\num{2177.8333333333335} \pm \num{56.31015302175384}\) & \(\num{1688.5333333333333} \pm \num{465.6906427153584}\) \\
\texttt{string\_utils.errors} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.1} \pm \num{0.5477225575051661}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.2} \pm \num{0.6643638388299197}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{string\_utils.manipulation} & \(\num{937.9} \pm \num{704.2264207796651}\) & \(\num{40787.066666666666} \pm \num{37729.391036636174}\) & \(\num{944.1} \pm \num{622.9696040628362}\) & \(\num{1694.9333333333334} \pm \num{30.97488786357296}\) & \(\num{444.7} \pm \num{64.18569504395711}\) \\
\rowcolor{gray!25}
 & \(\num{3599.6666666666665} \pm \num{1175.772771072456}\) & \(\num{170244.76666666666} \pm \num{3494.4030093785723}\) & \(\num{3605.5} \pm \num{1037.95411333031}\) & \(\num{1983.3} \pm \num{375.17850004571386}\) & \(\num{516.0} \pm \num{104.43014494107433}\) \\
\texttt{string\_utils.validation} & \(\num{2190.5666666666666} \pm \num{618.2867699417944}\) & \(\num{158014.13333333333} \pm \num{6162.930347194248}\) & \(\num{1705.6333333333334} \pm \num{446.37764152181137}\) & \(\num{1466.4} \pm \num{36.48580262380764}\) & \(\num{460.6666666666667} \pm \num{56.55106531716044}\) \\
 & \(\num{2713.0333333333333} \pm \num{673.8915539141158}\) & \(\num{164123.66666666666} \pm \num{2783.5272504545355}\) & \(\num{2392.9} \pm \num{490.91212430851965}\) & \(\num{1817.2333333333333} \pm \num{52.402739684455256}\) & \(\num{511.8} \pm \num{67.94439917543127}\) \\
\rowcolor{gray!25}
\texttt{sty.lib} & \(\num{0.4666666666666667} \pm \num{1.525266134682468}\) & \(\num{39.56666666666667} \pm \num{24.93257574606629}\) & \(\num{1.6333333333333333} \pm \num{7.1894718684425225}\) & \(\num{764.4} \pm \num{465.76223029826474}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{33.3} \pm \num{37.92201616930233}\) & \(\num{649.6666666666666} \pm \num{533.7062561148144}\) & \(\num{35.03333333333333} \pm \num{39.302964118571865}\) & \(\num{1427.5333333333333} \pm \num{503.32376180288003}\) & \(\num{24.766666666666666} \pm \num{27.28101946387828}\) \\
\texttt{sty.register} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{sty.renderfunc} & \(\num{0.0} \pm \num{0.0}\) & \(\num{2.5} \pm \num{1.9608231909600866}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{12.3} \pm \num{4.87887776807967}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{2.0} \pm \num{1.2865350418053538}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{9.766666666666667} \pm \num{4.6064672179323125}\) & \(\num{0.0} \pm \num{0.0}\) \\
\texttt{thonny.languages} & \(\num{6807.6} \pm \num{423.0373424456147}\) & \(\num{499907.4} \pm \num{17524.699630659223}\) & \(\num{6873.466666666666} \pm \num{409.91965010259}\) & \(\num{2011.6} \pm \num{52.506551315378566}\) & \(\num{1980.3} \pm \num{737.2160657407072}\) \\
 & \(\num{7144.633333333333} \pm \num{1005.7798649712615}\) & \(\num{561372.8666666667} \pm \num{12707.41034344849}\) & \(\num{7000.066666666667} \pm \num{1057.1129823586807}\) & \(\num{2030.8333333333333} \pm \num{55.879848525782236}\) & \(\num{1908.7} \pm \num{556.2564621864074}\) \\
\rowcolor{gray!25}
\texttt{thonny.plugins.pgzero\_frontend} & \(\num{7875.9} \pm \num{408.72521331574336}\) & \(\num{915035.1333333333} \pm \num{9758.948698796768}\) & \(\num{7974.466666666666} \pm \num{406.71499241787393}\) & \(\num{4076424.1333333333} \pm \num{59043.64307149435}\) & \(\num{3187.0666666666666} \pm \num{1581.463637514821}\) \\
\rowcolor{gray!25}
 & \(\num{7902.1} \pm \num{447.5005952606328}\) & \(\num{912116.8333333334} \pm \num{10778.095683258303}\) & \(\num{7743.7} \pm \num{473.8746487823765}\) & \(\num{4077571.8666666667} \pm \num{56390.235097890865}\) & \(\num{3354.5333333333333} \pm \num{1618.6520090608672}\) \\
\texttt{thonny.roughparse} & \(\num{2221.1} \pm \num{632.4151490039238}\) & \(\num{74916.63333333333} \pm \num{9800.573190427156}\) & \(\num{846.7333333333333} \pm \num{266.5591651130141}\) & \(\num{3501.2} \pm \num{388.57044805729663}\) & \(\num{773.8} \pm \num{178.50053607569458}\) \\
 & \(\num{2164.766666666667} \pm \num{829.296988661058}\) & \(\num{76400.36666666667} \pm \num{10547.3849005443}\) & \(\num{818.9333333333333} \pm \num{277.361078408799}\) & \(\num{3394.4} \pm \num{293.9915082048319}\) & \(\num{763.3333333333334} \pm \num{170.09334827216725}\) \\
\rowcolor{gray!25}
\texttt{thonny.terminal} & \(\num{549.7333333333333} \pm \num{159.95730752261696}\) & \(\num{78891.06666666667} \pm \num{1801.5304017711571}\) & \(\num{406.76666666666665} \pm \num{102.61500976896635}\) & \(\num{11144.266666666666} \pm \num{152.64765228173815}\) & \(\num{791.1666666666666} \pm \num{144.6334447260845}\) \\
\rowcolor{gray!25}
 & \(\num{472.3333333333333} \pm \num{76.31393117874364}\) & \(\num{85234.0} \pm \num{3156.50413350396}\) & \(\num{346.0} \pm \num{42.158158698258944}\) & \(\num{11267.7} \pm \num{136.11662089090598}\) & \(\num{896.8666666666667} \pm \num{181.2732236409873}\) \\
\texttt{thonny.token\_utils} & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
 & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) & \(\num{1.0} \pm \num{0.0}\) & \(\num{0.0} \pm \num{0.0}\) \\
\rowcolor{gray!25}
\texttt{typesystem.tokenize.positional\_validation} & \(\num{6433.233333333334} \pm \num{842.5576695020832}\) & \(\num{542453.9} \pm \num{8773.531001314948}\) & \(\num{5425.733333333334} \pm \num{540.9592969157109}\) & \(\num{14410.5} \pm \num{147.44999152254977}\) & \(\num{2176.8333333333335} \pm \num{900.4672382304849}\) \\
\rowcolor{gray!25}
 & \(\num{10383.766666666666} \pm \num{149.50508775412231}\) & \(\num{607153.4666666667} \pm \num{12625.352211497617}\) & \(\num{6260.766666666666} \pm \num{113.41066158399545}\) & \(\num{12050.8} \pm \num{119.6784196834627}\) & \(\num{4159.466666666666} \pm \num{2586.112122983781}\) \\
\texttt{typesystem.tokenize.tokenize\_yaml} & \(\num{5416.2} \pm \num{1085.6358505502662}\) & \(\num{363867.0333333333} \pm \num{10791.6289700136}\) & \(\num{5701.333333333333} \pm \num{626.9248612147994}\) & \(\num{2028.1333333333334} \pm \num{66.68026298136779}\) & \(\num{1512.2666666666667} \pm \num{448.70518186208307}\) \\
 & \(\num{5035.5} \pm \num{297.92521047149194}\) & \(\num{310418.1666666667} \pm \num{8046.379614603007}\) & \(\num{4897.233333333334} \pm \num{785.6905016403189}\) & \(\num{3545.4666666666667} \pm \num{269.40800148541956}\) & \(\num{1504.2} \pm \num{412.046733204897}\) \\
\rowcolor{gray!25}
\texttt{typesystem.unique} & \(\num{1.5} \pm \num{2.345207879911715}\) & \(\num{71.43333333333334} \pm \num{29.633023672146976}\) & \(\num{2.9} \pm \num{5.371380096207215}\) & \(\num{331.26666666666665} \pm \num{256.7668919109495}\) & \(\num{2.2} \pm \num{2.6444476641211603}\) \\
\rowcolor{gray!25}
 & \(\num{3.6666666666666665} \pm \num{3.8086411128428446}\) & \(\num{130.53333333333333} \pm \num{68.07588733745314}\) & \(\num{3.1} \pm \num{3.3768992102018784}\) & \(\num{537.1666666666666} \pm \num{278.7287747704881}\) & \(\num{2.1333333333333333} \pm \num{1.332183412176477}\) \\
\end{longtable}

==> generated/tables/coverage-effect-comparison.tex <==
\begin{tabular}{@{} l S[table-number-alignment=right,round-mode=places,round-precision=1] r S[table-number-alignment=right,round-mode=places,round-precision=1] r @{}} \toprule
Algorithm & \multicolumn{2}{c}{With Type Hints} & \multicolumn{2}{c}{Without Type Hints} \\
 & {median (\%)} & {mean (\%)} & {median (\%)} & {mean (\%)} \\ \midrule
DynaMOSA & 80.7207498383969 & \(\num[round-mode=places,round-precision=1]{71.59005093832216} \pm  \num[round-mode=places,round-precision=1]{30.501601017692202}\) & 76.47058823529412 & \(\num[round-mode=places,round-precision=1]{69.40724385009968} \pm  \num[round-mode=places,round-precision=1]{31.024142875254217}\) \\
MIO & 80.0 & \(\num[round-mode=places,round-precision=1]{71.3231377723311} \pm  \num[round-mode=places,round-precision=1]{30.72702253939233}\) & 75.0 & \(\num[round-mode=places,round-precision=1]{68.43210778861251} \pm  \num[round-mode=places,round-precision=1]{31.34696541514621}\) \\
MOSA & 80.0 & \(\num[round-mode=places,round-precision=1]{71.28297523262947} \pm  \num[round-mode=places,round-precision=1]{30.819930868767937}\) & 76.74418604651163 & \(\num[round-mode=places,round-precision=1]{68.73565466000007} \pm  \num[round-mode=places,round-precision=1]{31.651875735181083}\) \\
Random & 71.42857142857143 & \(\num[round-mode=places,round-precision=1]{66.93970907666117} \pm  \num[round-mode=places,round-precision=1]{31.508764298473306}\) & 66.66666666666666 & \(\num[round-mode=places,round-precision=1]{62.622772761835066} \pm  \num[round-mode=places,round-precision=1]{32.90571525287129}\) \\
WS & 80.0 & \(\num[round-mode=places,round-precision=1]{70.63297669822799} \pm  \num[round-mode=places,round-precision=1]{30.714453301022658}\) & 71.42857142857143 & \(\num[round-mode=places,round-precision=1]{67.50810878730078} \pm  \num[round-mode=places,round-precision=1]{31.487199600297462}\) \\
\bottomrule \end{tabular}

==> generated/tables/significant-mutation-scores.tex <==
\begin{tabular}{@{} l S[round-mode=figures] l S[round-mode=figures] @{}} \toprule
Module & {\effectsize} & Effect & {\pvalue} \\ \midrule
\verb!flutes.math! & 0.7138888888888889 & medium & 0.0024107506214976863 \\
\verb!flutils.strutils! & 0.8222222222222222 & large & 2.368621536405317e-06 \\
\verb!httpie.output.processing! & 0.7966666666666666 & large & 2.2414826823694543e-06 \\
\verb!httpie.output.streams! & 0.01 & large & 1.4966910378107542e-11 \\
\verb!httpie.plugins.base! & 0.8494444444444444 & large & 4.140113350008865e-08 \\
\verb!httpie.plugins.manager! & 0.3322222222222222 & medium & 0.008332851163536293 \\
\verb!httpie.status! & 0.6861111111111111 & medium & 0.011815893827992375 \\
\verb!isort.exceptions! & 0.8166666666666667 & large & 3.015756043532314e-07 \\
\verb!isort.utils! & 0.4 & small & 0.010891601176960192 \\
\verb!mimesis.providers.development! & 0.8161111111111111 & large & 2.005031368817652e-05 \\
\verb!mimesis.providers.transport! & 0.6477777777777778 & small & 0.013673478556222099 \\
\verb!mimesis.shortcuts! & 0.16666666666666666 & large & 5.853451971159792e-06 \\
\verb!py_backwards.files! & 0.0 & large & 7.255600677576213e-13 \\
\verb!py_backwards.transformers.class_without_bases! & 0.75 & large & 1.0174599213407037e-05 \\
\verb!py_backwards.transformers.dict_unpacking! & 1.0 & large & 7.82346679379162e-13 \\
\verb!py_backwards.utils.helpers! & 0.7838888888888889 & large & 2.8368107949719147e-05 \\
\verb!pymonet.monad_try! & 0.6133333333333333 & small & 0.015503350955664833 \\
\verb!pymonet.semigroups! & 0.6505555555555556 & small & 0.038248676162002934 \\
\verb!pypara.accounting.journaling! & 0.415 & small & 0.0437257609650295 \\
\verb!sanic.headers! & 0.6561111111111111 & small & 0.03830501161994476 \\
\verb!sanic.mixins.routes! & 0.345 & small & 0.035235925627921806 \\
\verb!string_utils.manipulation! & 0.7061111111111111 & medium & 0.0061361498803824506 \\
\verb!typesystem.tokenize.tokenize_yaml! & 0.9655555555555555 & large & 1.075531013945652e-10 \\
\bottomrule
\end{tabular}
